Random Walk Graph Laplacian based Smoothness Prior for Soft Decoding of JPEG Images

Given the prevalence of JPEG compressed images, optimizing image reconstruction from the compressed format remains an important problem. Instead of simply reconstructing a pixel block from the centers of indexed DCT coefficient quantization bins (hard decoding), soft decoding reconstructs a block by selecting appropriate coefficient values within the indexed bins with the help of signal priors. The challenge thus lies in how to define suitable priors and apply them effectively. In this paper, we combine three image priors---Laplacian prior for DCT coefficients, sparsity prior and graph-signal smoothness prior for image patches---to construct an efficient JPEG soft decoding algorithm. Specifically, we first use the Laplacian prior to compute a minimum mean square error (MMSE) initial solution for each code block. Next, we show that while the sparsity prior can reduce block artifacts, limiting the size of the over-complete dictionary (to lower computation) would lead to poor recovery of high DCT frequencies. To alleviate this problem, we design a new graph-signal smoothness prior (desired signal has mainly low graph frequencies) based on the left eigenvectors of the random walk graph Laplacian matrix (LERaG). Compared to previous graph-signal smoothness priors, LERaG has desirable image filtering properties with low computation overhead. We demonstrate how LERaG can facilitate recovery of high DCT frequencies of a piecewise smooth (PWS) signal via an interpretation of low graph frequency components as relaxed solutions to normalized cut in spectral clustering. Finally, we construct a soft decoding algorithm using the three signal priors with appropriate prior weights. Experimental results show that our proposal outperforms state-of-the-art soft decoding algorithms in both objective and subjective evaluations noticeably.

==> graph_xm.tex <==


Given that the sparsity prior is not sufficient to recover high frequency components of the original signal when QP is large and the dictionary is  small, in this section we introduce the graph-signal smoothness prior, which has been shown to restore piecewise smooth signals well \cite{jiahao,jiahao15,hu16spl}.
We first show how to define a discrete signal on a graph.
We then describe how smoothness can be defined for signals on a graph, and how graph-signal smoothness can be interpreted in the frequency domain.
Finally, we demonstrate how the smoothness prior can promote piecewise smooth signals during soft decoding.


%\subsection{Total-variation Prior}
%
%Given the observation that natural images tend to be smooth, one can use the popular total-variation (TV) prior \cite{DicTV} for further regularization. TV prior is defined as \cite{TV}:
%\begin{equation}
%p(\x) \propto \exp ( - (\left\| {\nabla_h\x} \right\|_1 + \left\| {\nabla_v\x} \right\|_1)),
%\end{equation}
%where $\nabla_h$ and $\nabla_v$ are first-order difference operators on horizontal and vertical directions, respectively.
%
%However, employing TV for soft decoding would encourage the smoothest signal possible within the q-bin constraints \red{again, this is not true in the general case. we should consider not saying this if this is confusing.}, potentially resulting in over-smoothing. As an pathological example, consider the q-bins for AC frequencies of a 1D 8-sample signal in Fig.~\ref{fig:smoothing}. Regardless of the q-bin sizes, TV norm would promote coefficient reconstructions closest to the zero q-bin boundaries, resulting in an almost DC signal. Assuming that each DCT coefficient takes on a Laplacian probability distribution (common in the image / video coding literature \cite{dctlaplacian}), the TV-reconstructed DC signal can be arbitrarily far from the minimum mean square error (MMSE) solution closer to the q-bin centers as the q-bin sizes increase.
%




%\begin{figure}[t!]
%\centering
%\includegraphics[width = 0.5\textwidth]{fig/smoothing2.png}
%\caption{Illustration of over-smoothing effect of TV. TV will choose the values indicated by $\times$, while MMSE will choose values indicated by red points. }
%\label{fig:smoothing}
%\end{figure}


\subsection{Signal on Graphs}

We first define a graph $\mathcal{G}$ as: $\mathcal{G} = \left(\VV, \E, \W\right)$.
$\VV$ and $\E$ are respectively the sets of vertices and edges in $\mathcal{G}$.
$W_{i,j}$ in the adjacency matrix $\mathbf{W}$ is the weight of the edge connecting vertices $i$ and $j$.
As done in \cite{shuman13} and others, we consider here only undirected graphs and non-negative edge weights; \textit{i.e.}, $W_{i,j} = W_{j.i}$ and $W_{i,j} \geq 0$.

A graph-signal $\x \in \mathbb{R}^n$ is a collection of discrete samples on vertices $\VV$ of a graph $\mathcal{G}$, where $n = |\VV|$.
In our work, for each target pixel patch we construct a fully-connected graph, where each vertex (pixel) is connected to all other vertices in $\mathcal{G}$.
The edge weight $W_{i,j}$ between two vertices $i$ and $j$ is conventionally computed using Gaussian kernels \cite{mao}:
\begin{equation}
W_{i,j} = \exp \left( - \frac{\left\| x_i - x_j \right\|_2^2 }{\sigma_1^2} \right) \;
\exp \left( - \frac{\left\| l_i - l_j \right\|_2^2 }{\sigma_2^2} \right)
\label{eq:weight}
\end{equation}
where $x_i$ and $l_i$ are the intensity and location of pixel $i$, and $\sigma_1$ and $\sigma_2$ are chosen parameters.
This definition is similar to weights used in bilateral filter \cite{BilateralFilter}.

\red{I think this can be discussed later.}
The computation of edges weights relies on values of pixels in $\x$. However, in soft decoding $\x$ is unknown. We propose to exploit an iterative strategy to set suitable edge weights: 1) compute edge weights based on some initial estimation, (i.e, the estimation based on Laplacian prior); 2) refine the estimation based on the proposed soft decoding method; these two steps are iteratively performed.
%\red{it's a restoration problem, so obviously we don't know $\x$. so how to find suitable edge weights?}


\subsection{Graph-signal Smoothness}

A \textit{degree matrix} $\mathbf{D}$ is a diagonal matrix where $D_{i,i} = \sum_j W_{i,j}$.
A \textit{combinatorial graph Laplacian} $\mathbf{L}$ is defined as \cite{graphoverview}:
\begin{equation}
\mathbf{L} = \mathbf{D} - \mathbf{W},
\end{equation}
the corresponding normalized graph Laplacian $\LL$ is defined as \cite{graphoverview}:
\begin{equation}
\LL = \mathbf{D}^{-1/2}\mathbf{L}\mathbf{D}^{-1/2}.
\end{equation}

Given $\LL$, one can describe the squared variations of the signal $\x$ with respect to $\mathcal{G}$ using the \textit{graph Laplacian regularizer} $\x^T \LL \x$ \cite{jiahao,jiahao15}:
\begin{equation}
\label{eq:GL}
\begin{array}{l}
\x^T\LL\x = \frac{1}{2}\sum\limits_{i = 1}^n {\sum\limits_{j = 1}^n {{{\left( {\frac{{{x_i}}}{{\sqrt {{d_j}} }} - \frac{{{x_j}}}{{\sqrt {{d_j}} }}} \right)}^2}{W_{i,j}}} }.
\end{array}
\end{equation}

Accordingly, the graph-signal smoothness prior is defined as:
\begin{equation}
\label{eq:graphprior}
\begin{array}{l}
P_G(\x) \propto \exp \left( { - \gamma{\x^T}\LL\x} \right),
\end{array}
\end{equation}
which states that a probable signal $\x$ has small $\x^T\LL\x$.
By (\ref{eq:GL}), $\x^T\LL\x$ is small if $\x$ has similar values at each pair of vertices $i$ and $j$ connected by an edge, \textit{or} the edge weight $W_{i,j}$ is small.
Thus a graph-signal $\x$ is smooth if its variations across connected vertices are consistent with the underlying graph structure (where edge weights reflect expected signal variations).
For example, if a discontinuity is expected at pixel pair $(x_i, x_j)$, as shown in Fig.~\ref{fig:smoothness}, one can pre-set a small weight $W_{i,j}$, so that the smoothness prior will not result in over-smoothing across this edge during optimization.

\begin{figure}[t!]
\centering
\includegraphics[width = 0.5\textwidth]{fig/smoothness.png}
\caption{Illustration of smoothing along edge. There is an edge (the black line) cross two pixels $x_i$ and $x_j$, a small edge weight $W_{i,j}$ is set in graph $\mathcal{G}$, so that employing the graph Laplacian regularizer as smoothness prior for optimization will not result in over-smoothing at this pair. }
\label{fig:smoothness}
\end{figure}


\subsection{Frequency Interpretation of Graph Smoothness Prior}

Since $\L$ is a real, symmetric, positive semi-definite matrix, it can be decomposed into a set of orthogonal eigenvectors, denoted by $\{\u_i\}_{i=0,\cdots, n-1}$, with real non-negative eigenvalues $0 = \eta_0 < \eta_1 \le \cdots \le \eta_{n-1}$.
We define $\U$ as the eigenmatrix with $\u_i$'s as columns and $\bm{\Lambda}$ as the diagonal matrix with $\eta_i$'s on its diagonal. $\L$ can thus be written as:
\begin{equation}
\label{eq:Ldec}
\begin{array}{l}
\L = \U\bm{\Lambda}\U^T,
\end{array}
\end{equation}

We define the \textit{graph Fourier transform} (GFT) matrix as $\FF = \U^T$. A graph-signal $\x$ can be transformed to its graph frequency domain as:
\begin{equation}
\label{eq:GFT}
\begin{array}{l}
\s = \FF\x,
\end{array}
\end{equation}
where eigenvalues $\eta_i$'s are interpreted as graph frequencies. $\eta_0 = 0$ is interpreted as the DC frequency.

With above definitions, the graph Laplacian regularizer can be written as:
\begin{equation}
\label{eq:graphfre}
\begin{array}{l}
\x^T\mathbf{L}\x =  \s^T\bm{\Lambda}\s = \sum\limits_{i}{{\eta_i}\s_i^2}.
\end{array}
\end{equation}
One can see that $\x^T\mathbf{L}\x$ is written as a sum of squared GFT coefficients $\s_i^2$, each scaled by the graph frequency $\eta_i$.
The eigenvalues of graph Laplacian are interpreted as frequencies in graph transform domain.
A smooth graph-signal with small $\x^T\mathbf{L}\x$ thus means that its energy resides mostly in the low frequencies in the GFT domain.

%\red{this discussion comes out of no where.}
%In graph definition, image similarity is embedded as edge weights into the graph, so that discontinuities in natural images will be interpreted as low graph frequencies. In contrast, DCT essentially assumes that every pair of adjacent pixels are equally similar. Thus, edge (discontinuities) common in natural images would translate to high DCT frequencies.



\subsection{Illustrative Example: 1-D Line Graph}

It is worth noting that the desirable property of the graph-signal smoothness prior on promoting low graph frequencies is only feasible for piecewise smooth (PWS) signal, assuming that its structure is appropriately described by the edge weights.
\red{what??}
1-D PWS signal is defined as consisting of two band-limited pieces with an abrupt discontinuity between them; a 2-D PWS signal is defined as consisting of two regions with an abrupt boundary between the regions. For an edge patch of natural images, it is highly probable to be PWS if the patch size is small.

We would like to show the principle of graph-signal smoothness prior on an illustrative example.
\red{what principle??}
For simplicity, we will consider 1-D PWS signal. We choose it because the relevant quantities can easily be plotted. The toy data set consists of nine samples $[5,5,5,5,1,1,1,1,1]$, which are connected to its immediate neighbor, with edge weights being 1 except for $W_{4,5} = W_{5,4} = 0.05$. It is easy to see there is a discontinuity between the fourth and fifth samples.

\begin{figure}[t!]
\centering
\includegraphics[width = 0.5\textwidth]{fig/rec_sign.png}
\caption{(a) Signal reconstruction comparison using only DC and 1st AC of GFT and DCT. (b) The sign consistency of 1st graph AC and the original data removed DC. }
\label{fig:rec}
\end{figure}

%\begin{figure}[htbp]
%\centering
%\includegraphics[width = 0.22\textwidth]{fig/GFTvsDCT.png}
%\includegraphics[width = 0.22\textwidth]{fig/sign.png}
%\caption{(a) Signal reconstruction using only DC and 1st AC component. (b) The sign consistency of 1st graph AC and the original data removed the mean.}
%\end{figure}

Fig.~\ref{fig:rec} (a) shows an example where a smooth graph-signal containing only DC and 1st graph AC components represents the original signal well. In contrast, the reconstruction by DCT, which also just uses DC and 1st AC, is poor. This is because that 1st graph AC components hold the same signs as those of the original data (the mean is removed), as illustrated in Fig.~\ref{fig:rec} (b), which will be explained later. In GFT, as shown in (\ref{eq:GFT}), there will be no items cancelled in the inner product between the 1st graph AC and the original data. It means that most energy concentrate in the low graph frequencies. By minimizing (\ref{eq:graphfre}), we suppress high graph frequencies and promote low graph frequencies, which are corresponding to signal discontinuities in graph. Therefore, the graph-signal smoothness prior is helpful to preserve signal structures, which are corresponding to high DCT frequencies. This means, when the dictionary size is limited, the graph-signal smoothness prior can act as an effective complement of the sparsity prior.
\red{not sure how important this 1-D example is in light of the analogy to spectral clustering.}



\subsection{Theoretical Analysis: A Spectral Clustering Perspective}

In this section, we provide intuition on why \textit{piecewise smooth} (PWS) signals on fully connected graphs can be well approximated using linear combinations of only low graph frequencies from a spectral clustering perspective.

\subsubsection{Analysis of Piecewise Constant Signals}

We start from the ideal case, where the target PWS signal is actually \textit{piecewise constant} (PWC).
Specifically, consider a PWC graph-signal $\x = [x_1,\cdots,x_N]^T$, where:
\begin{equation}
x_n = \left\{ \begin{array}{ll}
c_1 & \mbox{if}~ 1 \leq n \leq l \\
c_2 & \mbox{if}~ l < n \leq N
\end{array} \right.
\label{eq:pwc_sig}
\end{equation}
where constants $c_1$ and $c_2$ are sufficiently different, \textit{i.e.}, $|c_1 - c_2| > \Delta$ for some sufficiently large $\Delta$.

Using (\ref{eq:weight}) to compute edge weights, this PWC signal implies that $W_{i,j} = 0$ if $i$ and $j$ belong to different constant pieces.
Assume further that $\sigma_2$ is sufficiently large relative to location differences $\| l_i - l_j\|^2$, so that the first exponential kernel in (\ref{eq:weight}) alone determines $W_{i,j}$.
The adjacency matrix $\mathbf{W}$ and the graph Laplacian $\mathbf{L}$ are then both block-diagonal:

\vspace{-0.1in}
\begin{small}
\begin{equation}
\mathbf{W} = \left[ \begin{array}{cc}
\mathbf{A}_{l} & \mathbf{0}_{l \times (N-l)} \\
\mathbf{0}_{(N-l) \times l} & \mathbf{A}_{N-l}
\end{array} \right],
~
\mathbf{L} = \left[ \begin{array}{cc}
\mathbf{B}_{l} & \mathbf{0}_{l \times (N-l)} \\
\mathbf{0}_{(N-l) \times l} & \mathbf{B}_{N-l}
\end{array} \right]
\end{equation}
\end{small}\noindent
where $\mathbf{0}_{n \times m}$ is a $n \times m$ matrix of all zeros, and $\mathbf{A}_n$ and $\mathbf{B}_n$ are $n \times n$ square adjacency and graph Laplacian matrices for full unweighted graph of $n$ vertices:

\vspace{-0.1in}
\begin{footnotesize}
\begin{equation}
\mathbf{A}_n = \left[ \begin{array}{cccc}
0 & 1 & \ldots & \\
1 & 0 & 1 & \ldots \\
\vdots & & \ddots &
\end{array} \right],
~
\mathbf{B}_n = \left[ \begin{array}{cccc}
n-1 & -1 & \ldots & \\
-1 & n-1 & -1 & \ldots \\
\vdots & & \ddots &
\end{array} \right]
\end{equation}
\end{footnotesize}

Clearly, the normalized graph Laplacian $\LL = \mathbf{D}^{-1/2}\L\mathbf{D}^{-1/2}$ is also block-diagonal:
\begin{equation}
\LL = \left[ \begin{array}{cc}
\tilde{\mathbf{B}}_{l} & \mathbf{0}_{l \times (N-l)} \\
\mathbf{0}_{(N-l) \times l} & \tilde{\mathbf{B}}_{N-l}
\end{array} \right]
\label{eq:normL_PWC}
\end{equation}
where $\tilde{\mathbf{B}}_n$ is a $n \times n$ normalized graph Laplacian for a full unweighted graph of $n$ vertices:

\vspace{-0.1in}
\begin{footnotesize}
\begin{equation}
\tilde{\mathbf{B}}_n = \left[ \begin{array}{cccc}
1 & -1/(n-1) & \ldots & \\
-1/(n-1) & 1 & -1/(n-1) & \ldots \\
\vdots & & \ddots &
\end{array} \right]
\label{eq:normL_full}
\end{equation}
\end{footnotesize}

From (\ref{eq:normL_PWC}) and (\ref{eq:normL_full}), it is clear that the all-one vector $\mathbf{1}$ is an (unnormalized) eigenvector $\mathbf{v}_1$ corresponding to eigenvalue $0$, \textit{i.e.}, $\mathcal{L} \mathbf{1} = \mathbf{0}$.
Further, corresponding to eigenvalue $0$ a second (unnormalized) eigenvector $\mathbf{v}_2$ can be constructed as:
\begin{equation}
v_{2,n} = \left\{ \begin{array}{ll}
1/l & \mbox{if}~ 1 \leq n \leq l \\
-1/(N-l) & \mbox{if}~ l < n \leq N
\end{array} \right.
\end{equation}
It is easy to verify that $\mathcal{L} \mathbf{v}_2 = \mathbf{0}$ and $\mathbf{v}_1^T \mathbf{v}_2 = 0$.

Given the PWC signal $\mathbf{x}$ defined in (\ref{eq:pwc_sig}), we can express it as a linear combination of these two eigenvectors, \textit{i.e.}, $\mathbf{x} = a_1 \mathbf{v}_1 + a_2 \mathbf{v}_2$, where $a_1 = c_1 \frac{l}{N} + c_2 \frac{N-l}{N}$ and $a_2 = \frac{l(c_1 - c_2)(N-l)}{N}$.
Because $\v_1$ and $\v_2$ are the first two graph frequencies of $\mathcal{L}$, this leads us to the following conclusion:

\begin{quote}
\textit{An ideal two-piece PWC signal on a complete graph can be represented exactly using the first two graph frequency components of the normalized graph Laplacian.}
\end{quote}
In other words, PWC signals are ideal low-pass graph-signals in the graph frequency domain.



\subsubsection{Analysis of Piecewise Smooth Signals}

We now generalize our analysis of PWC signals to PWS signals. We first define a PWS signal $\mathbf{x}$ as:
\begin{equation}
\begin{array}{ll}
|x_i - x_j| \leq \delta & \mbox{if}~~ i,j \leq l ~~\mbox{or}~~ i,j > l \\
|x_i - x_j| > \Delta & \mbox{if}~~ i \leq l < j ~~\mbox{or}~~ j \leq l < i
\end{array}
\label{eq:pws_sig}
\end{equation}
where $\delta \ll \Delta$.
In words, $\mathbf{x}$ contains two smooth pieces in $[1, l]$ and $[l+1, N]$: two samples in the same piece are similar to within $\delta$, and two samples from two different pieces differ by more than $\Delta$.
Clearly, if $\delta = 0$, then $\mathbf{x}$ is PWC.

We now construct a complete graph for $\mathbf{x}$ using (\ref{eq:weight}) to compute edge weight $W_{i,j}$ between vertices $i$ and $j$.
The resulting normalized graph Laplacian $\mathcal{L}$ is still block-diagonal (for sufficiently large $\Delta$), but the diagonal blocks are not $\tilde{B}_n$ in (\ref{eq:normL_PWC}) corresponding to full unweighted graphs.

To understand low graph frequencies for $\mathcal{L}$ computed from this PWS signal $\mathbf{x}$, we take a \textit{spectral clustering} perspective.
Spectral clustering \red{add refs} is the problem of separating vertices $\mathcal{N}$ in a similarity graph $\mathcal{G}=(\mathcal{N}, \mathcal{E}, \mathbf{W})$ into two subsets of roughly the same size via spectral graph analysis.
Specifically, in a landmark paper by Shi and Malik \red{add ref}, the authors proposed a minimization objective \textit{normalized cut} (Ncut) to divide $\mathcal{N}$ into subsets $\mathcal{A}$ and $\mathcal{B}$:
\begin{equation}
\mathrm{Ncut}(\mathcal{A}, \mathcal{B}) := \mathrm{cut}(\mathcal{A}, \mathcal{B})
\left( \frac{1}{\mathrm{vol}(\mathcal{A})} + \frac{1}{\mathrm{vol}(\mathcal{B})} \right)
\label{eq:ncut}
\end{equation}
where $\mathrm{cut}(\mathcal{A}, \mathcal{B})$ counts the edges across the two subsets $\mathcal{A}$ and $\mathcal{B}$, and $\mathrm{vol}(\mathcal{A})$ counts the degrees of vertices in $\mathcal{A}$:
\begin{equation}
\mathrm{cut}(\mathcal{A},\mathcal{B}) =
\sum\limits_{i \in \mathcal{A}, j \in \mathcal{B}} {{W_{i,j}}},~~
\mathrm{vol}(\mathcal{A}) =  \sum\limits_{i \in \mathcal{A}} D_i
\end{equation}
From (\ref{eq:ncut}) it is clear that a division of $\mathcal{N}$ into clusters $\mathcal{A}$ and $\mathcal{B}$ with small $\mathrm{Ncut}(\mathcal{A}, \mathcal{B})$ will have small $\mathrm{cut}(\mathcal{A}, \mathcal{B})$ and large $\mathrm{vol}(\mathcal{A})$ and $\mathrm{vol}(\mathcal{B})$.
However, minimizing Ncut over all possible $\mathcal{A}$ and $\mathcal{B}$ that divide $\mathcal{N}$ is NP-hard.

Towards an approximation, the authors first rewrote the minimization of Ncut as:
\begin{equation}
\min_{\mathcal{A}, \mathcal{B}} \mathrm{Ncut}(\mathcal{A}, \mathcal{B}) =
\min_{\mathbf{f}} \frac{{{\f^T}\L\f}}{{{\f^T}\D\f}}
\label{eq:relaxed_ncut}
\end{equation}
where
\begin{equation}
\f= [f_1,\cdots,f_n]^T \hspace{0.2cm} \mbox{and} \hspace{0.2cm}
{f_i} = \left\{ \begin{array}{ll}
\frac{1}{\mathrm{vol}(\mathcal{A})}  & \mbox{if} \hspace{0.2cm} i \in \mathcal{A} \\
\frac{{ - 1}}{\mathrm{vol}(\mathcal{B})} & \mbox{if} \hspace{0.2cm} i\in \mathcal{B}
\end{array} \right.
\label{eq:relaxed_ncut2}
\end{equation}

The constraints in problem (\ref{eq:relaxed_ncut}) are then relaxed to:
\begin{equation}
\min_{\mathbf{f}} \frac{{{\f^T}\L\f}}{{{\f^T}\D\f}},
\hspace{0.2cm}\mbox{s.t.} \hspace{0.2cm} \f^T\D\mathbf{1} = 0
\label{eq:relaxed_ncut3}
\end{equation}
The observation is that if solution $\mathbf{f}$ satisfies (\ref{eq:relaxed_ncut2}), then $\mathbf{f}^T \mathbf{D} \mathbf{1} = 0$.
Thus a solution $\mathbf{f}$ to (\ref{eq:relaxed_ncut3}) can be interpreted as an approximate solution to the Ncut problem in (\ref{eq:ncut}).

We now use this result from \red{add ref} to interpret low graph frequencies derived from the normalized graph Laplacian $\mathcal{L}$.
We first define $\v := \D^{1/2}\f$ and $\mathbf{v}_1 := \D^{1/2} \mathbf{1}$.
(\ref{eq:relaxed_ncut3}) can then be rewritten as:
\begin{equation}
\min_{\mathbf{v}}
\frac{{{\v^T}\LL\v}}{{{\v^T}\v}},\hspace{0.2cm}\mbox{s.t.}
\hspace{0.2cm} \v^T \v_1 = 0
\label{eq:relaxed_cut4}
\end{equation}
Note that the objective in (\ref{eq:relaxed_cut4}) is the \textit{Rayleigh quotient} with respect to matrix $\mathcal{L}$ \cite{MatrixAnalysis}.
It is easy to see that $\v_1$ minimizes this objective:
$\v_1^T \mathcal{L} \v_1 = \mathbf{1}^T \D^{1/2} \D^{-1/2} \mathbf{L} \D^{-1/2} \D^{1/2} \mathbf{1} = \mathbf{1}^T \mathbf{L} \mathbf{1} = 0$.
Hence $\v_1$ is the first eigenvector of $\mathcal{L}$, and the solution to (\ref{eq:relaxed_cut4}) is the second eigenvector $\v_2$ of $\mathcal{L}$.





The above analysis shows that the second eigenvector $\v_2$ of $\mathcal{L}$ is related to the approximate solution $\mathbf{f}^*$ of Ncut via $\v_2 = \D^{1/2} \mathbf{f}^*$.



==> system.tex <==
\subsection{System Overview}

\begin{figure*}[htbp]
\centering
\includegraphics[scale=0.19]{fig/system_ming_new.eps}
%\includegraphics[scale=0.5]{fig/system_ming.png}
\caption{Block diagram of the proposed joint gaze correction and face
beautification system}
\label{fig:system}
\end{figure*}

We first overview our proposed joint gaze correction / face beautification system, as illustrated in Fig.\,\ref{fig:system}. Towards the goal of low-cost deployment, our proposed system employs a single depth-sensing camera that is capable
of capturing texture (color) and depth images simultaneously, such as MS Kinect$^{\textregistered}$, at the bottom of a large display. Prior to the start of a video conference session, we assume a large image collection of ``beautiful'' people in frontal views with various expressions is available for offline dictionary training. Two dictionaries are trained; the first operates per pixel patch and is used for image completion, and the second operates per facial component (\textit{e.g.}, eyes or eyebrows) and is used for facial component beautification. In general, it is difficult to mathematically define the notion of human facial beauty. Thus, we simply gather images of television and movies stars in China, Japan and South Korea publicly available on the Internet, male and female, with ages from twenties to forties. \textcolor[rgb]{1.00,0.00,0.00}{The assumption here is that if the dictionaries are trained using facial components of young and popular TV and movie stars, then reconstructing facial components like eyes and eyebrows that are similar to them will also be beautiful.} We will demonstrate via extensive experimentation that this is indeed the case in Section~\ref{sec:results}.

During a video conference session, each pair of texture and depth images captured at the same time instant are processed as follows. First, foreground / background segmentation is performed by thresholding the depth image; \textit{i.e.}, depth pixels with values smaller than a pre-selected value $\tau$ are deemed foreground. This simple thresholding method has been shown to be effective for conference video in \cite{lee11,lee13} as well. Second, assuming that the center of the display monitor is the desired virtual viewpoint, DIBR is performed only for the classified foreground pixels, so that texture pixels from the captured camera viewpoint can be mapped to the virtual view given corresponding available depth pixels. The necessary intrinsic and extrinsic matrices needed for DIBR to map from captured to virtual view can be derived using standard camera calibration tools \cite{calibration}. Due to self-occlusion, insufficient pixel sampling and missing depth pixels in the captured texture / depth image pair, there will be missing pixels in the DIBR-synthesized foreground that requires filling. Further, depth errors due to sensing and / or compression noise and synthesis errors due to rounding to the nearest pixel grid means that the actual rendered pixels are also corrupted by noise.

To fill in the missing pixels in the DIBR-synthesized image, one conventional method is inpainting, where information from neighboring available pixels is methodically propagated into the hole regions based on detected image structure~\cite{oh09, reel13, bruno14}. To simultaneously denoise the DIBR-rendered pixels also, one can optimize an image reconstruction objective that trades off fidelity (difference between observed and reconstructed pixels) and signal prior like sparsity in a chosen dictionary \cite{mao13icassp, mao14}. This joint hole-filling / denoising problem is clearly an inverse imaging problem, whose success depends heavily on the appropriateness of the signal prior(s) used for regularization of the ill-posed problem. In this paper, we perform joint denoising / hole-filling of DIBR-rendered human faces with the aid of dictionaries trained offline using beautiful human facial images. The key insight in our approach is the following: \textit{given that the joint denoising / hole-filling problem for facial images is inherently ill-posed, we use beautiful facial components learned offline as signal priors, so that even when the rendered faces are incorrect, they err on the side of human perceptual beauty.} The amount beautification applied to our optimization can be tuned simply by adjusting the strength of the signal prior.

Finally, the reconstructed gaze-corrected / beautified face is transposed and warped into the original captured view, replacing the gaze-mismatched face. By reusing the background of the captured image, also done in \cite{kuster12}, there is no need to complete missing background pixels due to occlusion in the virtual view.


\subsection{Joint Face Restoration / Beautification Optimization}

The key technical contribution in our system is the joint gaze-corrected face image restoration / face component beautification process via a unified dual sparse coding framework. Given the two offline trained dictionaries $\bm{\Phi}$ and $\bm{\Psi}$, we jointly search for two sparse code vectors $\a$ and $\b$ for the two dictionaries that respectively explain the observed DIBR-synthesized pixels and achieve proximity to beautiful facial components. We illustrate the joint optimization geometrically in Fig.\,\ref{fig:2dplots}. Given an incomplete and noise-corrupted observation $\mathbf{x}$, we seek a sparse face reconstruction $\bm{\Phi} \a$ that is close to $\mathbf{x}$ in a $l_2$-norm sense (fidelity term), resulting in a circle for a 2-dimensional space. At the same time, to maintain a desired level of recognizability of the conference subject, we enforce a feature space distance constraint $S$ to restrict the amount of beautification performed; mathematically it means beautification $\bm{\Psi} \b$ must be close to reconstructed $\bm{\Phi} \a$ in a defined feature space, resulting in a blue region for given $\a$.


\begin{figure*}[htbp]
\begin{center}
\includegraphics[scale=0.45]{fig/2dplots.eps} \\
\end{center}
\vspace{-0.2in}
\caption{Search space for dual code vectors. On the left, given
observation $\mathbf{x}$, a face reconstruction $\bm{\Phi} \a$ must be
close in $l_2$-norm sense (inside black circle), and beautification
$\bm{\Psi} \b$ must be close to $\bm{\Phi} \a$ in feature space
distance (blue region). If solved separately, search region for
$\b$ is only one blue region given one $\a$, rather the
union of all blue regions with center inside the circle.
On the right, an irregular-shaped blue region can be approximated
by a quadratic function.}
\label{fig:2dplots}
\end{figure*}

By jointly performing disocclusion hole-filling and facial components beautification simultaneously, we can potentially identify optimal pair of code vectors $\a$ and $\b$ that can minimize an overall objective function that considers fidelity of hole-filling, amount of beautification and sparsity of both vectors. Geometrically, the search space for this pair of vectors is the entire circle for $\a$ and the union of all blue regions with center inside the circle for $\b$. In contrast, if hole-filling and face beautification are performed in separate steps, then after solving for a fixed $\a$, only one blue region centered at $\bm{\Phi} \a$ is considered as search space for $\b$, which is much more restrictive.
%Further, we perform facial contours adjustment in the third step. We
%extract a set of distances between a variety of landmarks along the face
%contour, and propose a sparse neighbor selection strategy to find closely
%related neighbors adaptively. The
%weighted average of selected distance vectors serves as a target to define a
%2D warp field which maps the test facial contour to the adjusted
%locations. After these three steps, we will get a gaze-corrected and
%beautified face.
We will show in the experimental section that indeed by performing joint optimization, we can reconstruct facial components with higher beauty score than separate optimization. In the next section, we will introduce the details of our joint sparse coding framework.

